Differentially Private Federated Learning without Noise Addition: When is it Possible?

Federated Learning (FL) with Secure Aggregation (SA) has gained significant attention as a privacy preserving framework for training machine learning models while preventing the server from learning information about users' data from their individual encrypted model updates. Recent research has extended privacy guarantees of FL with SA by bounding the information leakage through the aggregate model over multiple training rounds thanks to leveraging the "noise" from other users' updates. However, the privacy metric used in that work (mutual information) measures the on-average privacy leakage, without providing any privacy guarantees for worse-case scenarios. To address this, in this work we study the conditions under which FL with SA can provide worst-case differential privacy guarantees. Specifically, we formally identify the necessary condition that SA can provide DP without addition noise. We then prove that when the randomness inside the aggregated model update is Gaussian with non-singular covariance matrix, SA can provide differential privacy guarantees with the level of privacy $\epsilon$ bounded by the reciprocal of the minimum eigenvalue of the covariance matrix. However, we further demonstrate that in practice, these conditions are almost unlikely to hold and hence additional noise added in model updates is still required in order for SA in FL to achieve DP. Lastly, we discuss the potential solution of leveraging inherent randomness inside aggregated model update to reduce the amount of addition noise required for DP guarantee.

==> docs/old/evaluation_old.tex <==
\vspace{-0.05in}
\section{Evaluation}
\label{sec:eval}
In this section, we start by numerically verifying our analytical results with simple models and datasets where the model update has a  non-singular covariance matrix. Then, we compare WF-DP with DDP under different large models and different datasets where the gradient update has a singular covariance matrix. We access the performance gain in terms of improving model accuracy for the same level of DP (i.e., $\epsilon$). Note that we use the algorithm proposed in \cite{gopi2021numerical} to calculate the $\epsilon$ across all training rounds.

\vspace{-0.05in}
\subsection{Verifying analytical results}
We use logistic regression and the UCI Wine dataset \cite{UCI_DATA} to evaluate our analytical results. Note that the UCI wine dataset contains 11 features indicating chemical properties of red and white wines as input and an integer value quality score as output. We randomly split the training dataset into 50 local datasets with equal size to simulate 50 users, and we use FedSGD to update the logistic regression model for 100 rounds. Since the model size is much smaller than the total number of training data points, we observe that the covariance matrix of the gradient update from each user is non-singular. Note that we focus on high privacy region where the $\epsilon^{(t)} \in (0,1)$ for each training round (see Appendix \ref{sec:appendix} for details on how we select FL parameters).

Figure \ref{fig:wine_user} shows how privacy provided by secure aggregation changes with the number of users without adding any noise. As we increase the number of users $N$ from 5 to 50, $\epsilon$ will decay at the rate of $O(\frac{1}{|\sqrt{\mathbb{U}_{s}}}|)$. This says, by aggregating more users, higher privacy can be achieved. Note that $\epsilon$ values in these experiments are not measured or estimated values. 
Specifically, we first set the number of users $N$. We then run federated learning with secure aggregation on the given dataset and compute the minimum eigenvalues of the covariance matrices and other parameters. Last, we report the $\epsilon$ across 100 training rounds for the given number of users, dataset and scenario.

Figure \ref{fig:wine_pu} shows the relationship between the provided privacy and the model performance/accuracy in terms of mean squared error (MSE). 
For a fixed number of users and thus $\epsilon$ values, we separate the dataset into a training and testing dataset, and evaluate the accuracy of the model on the testing dataset.
We observe that increasing the number of can reduce the MSE, meaning that the model performance is enhanced. This occurs because throughout this experiment we do not add any noise to the model updates for privacy reasons, privacy occurs from the aggregation of more users, and, at the same time, the more the users are, the larger and the more diverse the dataset is which improves accuracy.

% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\textwidth]{docs/fig/wine_cmp.png}
%   \caption{Description of the figure.}
%   \label{fig:test}
% \end{figure}

\begin{figure}
  \centering
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\textwidth]{docs/fig/wine_vary_user.png}
    \caption{$\epsilon$ vs $N$.}
    \label{fig:wine_user}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\textwidth]{docs/fig/wine_trade.png}
    \caption{$\epsilon$ vs MSE.}
    \label{fig:wine_pu}
  \end{subfigure}
  \vspace{-0.1in}
  \caption{Privacy provided by SA on UCI Wine dataset.}
  \label{fig:wine_sa}
  \vspace{-0.18in}
\end{figure}

\vspace{-0.05in}
\subsection{Comparison of WF-DP with DDP}
\label{subsec:exp_cmp}
For many of the real world FL applications, we use deep neural network models, where the covariance matrix of model update is typically singular due to over-parameterization \cite{du2018gradient, allen2019convergence}. In this case, WF-DP can be used to reduce the amount of noise added in model update for achieving the same level of DP, compared with DDP (as discussed in Section \ref{subsec:intuitive_cmp}).

For the same level of DP, to evaluate whether the amount of noise reduced by WF-DP can provide improvement in model accuracy, we compare it with DDP in three datasets: MNIST, FEMNIST, and Yelp Review, and we consider three different models: linear model, convolutional neural network (CNN) model, and pre-trained Bert model with one fully-connected neural network (FCNN) layer. Note that we use the DDP in \cite{stevens2022efficient} for FL with SA, where we distribute the Gaussian noise with scale $\sigma^2$ into $N$ users, such that each user only needs to add Gaussian noise with scale $\frac{\sigma^2}{N}$. By using the most efficient implementation of DDP in FL with SA, we ensure that the reported gains by WF-DP are over the best possible alternatives.

\noindent\textbf{MNIST.} We first conduct experiments on MNIST dataset, which contains 60,000 training images
and 10,000 testing images, with 10 classes of labels \cite{MNIST}. We randomly split the training dataset into 50 local datasets with equal size to simulate 50 users, and we consider the task of training both a simple linear model and a large CNN model using FedSGD with DP noise. Note that we use FedSGD to train models on MNIST dataset, since it can already make the model converge within 100 training rounds and it typically has better privacy-accuracy tradeoff compared with FedAvg \cite{li2020secure}. 

Specifically, we first set the number of users $N$ from $\{10, 20, 50\}$ and set $\sigma$ from $\{0.05, 0.1, 0.2\}$ in Eq. (\ref{eq:wfdp}). Then, for each model and each DP mechanism, we train the model for 100 rounds using FedSGD with DP noise. After training, we evaluate the model accuracy on the testing dataset, and report the $\epsilon$ across 100 training rounds.

%Moreover, we choose $\sigma$ in Eq. (\ref{eq:wfdp}) of Algorithm \ref{algo1} from $\{0.05, 0.1, 0.2\}$, corresponding to $\epsilon$ (i.e. the privacy budget) from $\{11.42, 2.28, 1.14\}$. Under each level of privacy and for each model, we train the model for 100 rounds until it converges with DP noise added by WF-DP and DDP separately, and then evalaute the model accuracy on testing dataset. 
As shown in Figure \ref{fig:mnist_lin}, for the same level of privacy and the linear model, WF-DP can achieve 1-2\% accuracy improvement compared with DDP. These results are consistent with the training of a CNN model, as demonstrated in Figure \ref{fig:mnist_cnn}. It is worth mentioning that 1-2\% accuracy is quite important in practice for large deep models in federated learning used in the industry. As a result, there is a sizable line of work on FL protocol varieties for even lower single digit performance gains, see, for example, \cite{liu2022unifed,chai2020fedeval,li2020federated}. 


\begin{figure}[!t]
  \centering
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\textwidth]{docs/fig/mnist_cmp_lin.png}
    \caption{Linear Model, MNIST dataset.}
    \label{fig:mnist_lin}
  \end{subfigure}
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\textwidth]{docs/fig/mnist_cmp_cnn.png}
    \caption{CNN model, MNIST dataset.}
    \label{fig:mnist_cnn}
  \end{subfigure}
  % \caption{Comparison of WF-DP with DDP on MNIST dataset.}
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\textwidth]{docs/fig/mnist_cmp_cnn_cf.png}
    \caption{CNN Model, CIFAR10 dataset.}
    \label{fig:cifar}
  \end{subfigure}
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.9\textwidth]{docs/fig/mnist_cmp_yelp.png}
    \caption{Bert model, Yelp dataset.}
    \label{fig:yelp}
  \end{subfigure}
  \vspace{-0.1in}
  \caption{Comparison of WF-DP with DDP. Note that $\epsilon=4.27/2.14/1.07$ represents $\sigma=0.05/0.1/0.2$.}
  \label{fig:cmp_all}
  \vspace{-0.15in}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{docs/fig/emnist_cmp_cnn.png}
    \caption{Comparison of WF-DP with DDP on CNN model, FEMNIST. Note that we report the average model accuracy across all users, and $\epsilon=72.09/13.02/3.33$ represents $\sigma=0.05/0.1/0.2$.}
    \label{fig:femnist}
    \vspace{-0.15in}
\end{figure}


\noindent\textbf{CIFAR10.} Next, we conduct experiments on CIFAR10, , which contains 50,000 training images
and 10,000 testing images, with 10 classes of labels \cite{CIFAR10}. We randomly split the training dataset into 50 local datasets with equal size to simulate 50 users, and we consider the task of training both a simple linear model and a large CNN model using FedSGD with DP noise.
Specifically, we set the number of users $N$ as 50 and set $\sigma$ from $\{0.05, 0.1, 0.2\}$ in Eq. (\ref{eq:wfdp}). Same as the experimental setup for the MNIST dataset, for each DP mechanism, we train the model for 100 rounds using FedSGD with DP noise. After training, we evaluate the model accuracy on the testing dataset, and report the $\epsilon$ across 100 training rounds.

%Moreover, we choose $\sigma$ in Eq. (\ref{eq:wfdp}) of Algorithm \ref{algo1} from $\{0.05, 0.1, 0.2\}$, corresponding to $\epsilon$ (i.e. the privacy budget) from $\{11.42, 2.28, 1.14\}$. Under each level of privacy and for each model, we train the model for 100 rounds until it converges with DP noise added by WF-DP and DDP separately, and then evalaute the model accuracy on testing dataset. 
As shown in Figure \ref{fig:cifar}, for the same level of privacy and the linear model, WF-DP can achieve 1-2\% accuracy improvement compared with DDP, which is consistent with our experimental results on MNIST dataset.

%Note that we do not evaluate use FedSGD on FEMNIST dataset, since we observe that it is hard and time-consuming for the model trained with FedSGD to converge to a reasonable accuracy.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{docs/fig/emnist_cmp_cnn.png}
%     \caption{Comparison of WF-DP and DDP on FEMNIST dataset.}
%     \label{fig:femnist}
%     \vspace{-0.2in}
% \end{figure}

\noindent\textbf{Yelp.} 
%Till now, we evaluate WF-DP on image classification datasets only. To evaluate WF-DP's performance on other types of FL tasks, 
Till now, we evaluate WF-DP in scenarios where the whole model can be trained on mobile devices. To analyze a practical scenario where the mobile device can not train the whole model due to limited resources, we consider the task of fine-tuning the last layer of a large transformer model on the Yelp review dataset. Specifically, we use a pre-trained Bert containing 110 millions of parameters \cite{devlin2018bert} with one FCNN layer. During the training process, we freeze the model parameters of Bert and only train the last FCNN layer during the training process. In the Yelp review dataset, each input is a Yelp review and the associated label is a binary sentiment polarity, indicating whether this review is positive or negative. We split the dataset into 50 local datasets to simulate 50 users.  

During our experiments, we set the number of users $N$ as 50 and select $\sigma$ in Eq. (\ref{eq:wfdp}) from $\{0.05, 0.1, 0.2\}$. Similar to the experimental setup for the MNIST dataset, for each DP mechanism, we train the model for 100 rounds using FedSGD with DP noise. After training, we evaluate the model accuracy on the testing dataset and calculate the $\epsilon$ across all the 100 training rounds.
%choose $\sigma$ from $\{0.01, 0.05\}$, which corresponds to $\epsilon$ from $\{6.90, 1.40\}$. Under each level of privacy, we train the model for 100 rounds until it converges with DP noise added by WF-DP and DDP separately and then compare the model accuracy. 
As shown in \ref{fig:yelp}, compared with DDP, the model trained with WF-DP can consistently achieve 1-3\% higher accuracy for the same level of DP (i.e. same $\epsilon$ values), which demonstrates that the performance gain of WF-DP can be preserved in FL tasks with large pre-trained models, which is an emerging application in FL \cite{liu2021federated, tan2022federated}.
%

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{docs/fig/mnist_cmp_yelp.png}
%     \caption{Comparison of WF-DP and DDP on Yelp dataset.}
%     \label{fig:yelp}
%     \vspace{-0.2in}
% \end{figure}
\noindent\textbf{FEMNIST.} So far, we evaluate WF-DP on datasets with homogeneous users only. To investigate whether WF-DP can be generalized to FL with heterogeneous users, we conduct experiments on FEMNIST, which is a benchmark FL dataset consisting of 62 classes of images written by 3600 with heterogeneous users \cite{caldas2018leaf}, each of which has hundreds of images. We consider the task of training a CNN model using FedAvg with DP noise, in order to evaluate the performance gain of WF-DP when it is applied to FL with FedAvg protocol and non-i.i.d user data distributions. 

Specifically, we first set the number of users participating in each training round as $50$, and select $\sigma$ in Eq. (\ref{eq:wfdp}) from $\{0.05, 0.1, 0.2\}$. Then, for each model and each DP mechanism, we train the model for 100 rounds using FedAvg protocol with DP noise until the model converges. Note that during each training round, we randomly select 50 out of 3600 users. Each user participating in this training round will divide their local dataset into batches with size 16, and iterate all these batches for one time to calculate the local model update. After training, we evaluate the model accuracy on the testing dataset, and calculate the $\epsilon$ across all the 100 training rounds.

%Similarly, we choose $\sigma$ in Eq. (\ref{eq:wfdp}) of Algorithm \ref{algo1} from $\{0.01, 0.025, 0.05\}$, which corresponds to $\epsilon$ from $\{22.27, 8.90, 4.45\}$. Under each level of privacy, we train the CNN model for 50 rounds until it converges with DP noise added by WF-DP and DDP separately, and then report the model accuracy on testing dataset. For each training round, we randomly select 50 of 3500 users to participate in FL. 
As demonstrated in Figure \ref{fig:femnist}, compared with DDP, WF-DP can achieve more than 5\% accuracy improvement for the same level of privacy. Hence, WF-DP can consistently outperform DDP on non-iid datasets and when using FedAvg for the same level of DP, by reducing the amount of added noise. 


\noindent\textbf{Remark 4: DDP baselines.}
We have implemented DDP using the vanilla Gaussian mechanism to add noise and Gaussian gradient descent for FL with SA, since WF-DP also uses the same. Note that both DDP and WF-DP could use other Gaussian mechanisms to add noise including recent works which propose methods to reduce the amount of noise added by the vanilla Gaussian mechanism \cite{zhang2021adaptive,andrew2021differentially}. In other words, WF-DP can be used in parallel with more efficient noise adding mechanisms. WF-DP's novelty is in deciding the directions of the covariance matrix space that may require additional noise (in addition to the inherent noise from other users) and it is orthogonal to which mechanism one may use to add this additional noise (see Section \ref{sec:related} for detailed discussion). In Section \ref{subsec:combine}, we demonstrate that WF-DP can be combined with the SOTA DPFL algorithm to further improve its performance.

% Theorem 4 + Proof: The proof follows by combining Theorems 2 and 3. 
% Add Theorem 5 for WF-DP + Proof: The proof follows by combining Theorems X and Y.
\vspace{-0.05in}
\subsection{Varying system parameters in WF-DP}
In this subsection, we investigate how different system parameters can affect the performance of WF-DP, including the number of users $N$ and the square root bound for minimum eigenvalues $\sigma$. Note that we use a linear model and the MNIST dataset for this case study, with the same experimental setup used for the MNIST dataset in Section \ref{subsec:exp_cmp}.

\noindent\textbf{Varying the number of users $N$.} We first fix the privacy level (we choose $\sigma=0.1$ per user), and change the number of users $N$ participating in FL. As shown in Figure \ref{fig:mnist_user}, by increasing the number of users $N$, $\epsilon$ will decay at the rate of $O(\frac{1}{N}|)$ in accordance to our theory (see Eq. (\ref{eq:wfdp_eps})). Recall that $\sigma$ captures the minimum standard deviation of noise contained in all eigenvector directions provided by each of the other users (see Eq. (\ref{eq:wfdp})). Hence, as more users participate in FL, the total amount of noise contained in aggregated model update from other users will increase. Hence, the privacy of each user will be enhanced. 


\noindent\textbf{Privacy-accuracy tradeoff.} Figure \ref{fig:mnist_trade} illustrates the privacy and accuracy tradeoff of WF-DP, with varying number of users and $\sigma$. 
%Note that $\sigma$ is the squared root of the lower bound for minimum eigenvalue value, in order to achieve the privacy budget $\epsilon$ (see Eq. (\ref{eq:wfdp}) in Algorithm  \ref{algo1}) 
For a fixed number of users $N$, we observe that the larger the $\sigma$ is, the higher privacy WF-DP can achieve. This is consistent with Eq. (\ref{eq:wfdp}), where $\epsilon$ is inversely proportional to $\sigma$. However, for a fixed number of users $N$, as we increase the $\sigma$ 
 the accuracy of the model trained with WF-DP will decrease, as more noise is added into the aggregated model update.

Moreover, for a fixed $\sigma$ value, larger $N$ will not change the model accuracy by much. This implies that the model accuracy mostly depends on $\sigma$, i.e., the amount of noise per user from the model update, and not on the number of users participating in FL. Note that a fixed $\sigma$ means the amount of noise contained in each user's model update is fixed. While increasing $N$ will increase the total noise in the aggregated model update (i.e. the sum of model updates from all users), it will not increase the amount of noise in the global model update, which will be the average sum of  model updates from all users (i.e. the aggregated model update divided by $N$). Hence, once $\sigma$ is fixed, the global model accuracy will not change much (see Figure \ref{fig:mnist_trade}). 

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{docs/fig/mnist_vary_user.png}
%     \caption{Comparison of WF-DP and DDP on FEMNIST dataset.}
%     \label{fig:mnist_user}
%     \vspace{-0.1in}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{docs/fig/mnist_trade.png}
%     \caption{Varying system parameters of WF-DP on MNIST dataset.}
%     \label{fig:mnist_trade}
%     \vspace{-0.15in}
% \end{figure}

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=0.85\linewidth]{docs/fig/mnist_vary_user.png}
        \caption{Varying $N$ when $\sigma=0.05$.}
        \label{fig:mnist_user}
    \end{subfigure}
    \begin{subfigure}{0.48\linewidth}
        \includegraphics[width=0.75\linewidth]{docs/fig/mnist_trade.png}
        \caption{Varying both $N$ and $\sigma$ }
        \label{fig:mnist_trade}
    \end{subfigure}
    \caption{Varying system parameters of WF-DP on MNIST dataset.}
    \label{fig:combined_figures}
    \vspace{-0.15in}
\end{figure}
\vspace{-0.05in}
\subsection{Combine WF-DP with PrivateFL}
\label{subsec:combine}
In this subsection, we demonstrate that WF-DP can be combined with other DPFL algorithms using Gaussian mechanisms, since the key novelty of WF-DP is leveraging the ``noise" from
other users’ updates to reduce the required noise added by DP mechanism. Specifically, we combine WF-DP with PrivateFL (PFL) \cite{yang2023privatefl}, which is the SOTA DPFL algorithm, and we compare PFL+WF-DP with PFL under the training of CNN model on MNIST dataset. As demonstrated in Figure \ref{fig:femnist}, when combining WF-DP with PFL, the testing accuracy of the CNN model after training can be increased by 0.5\%-6\%. Hence,  we conclude that WF-DP can be effectively combined with SOTA DPFL algorithm to further improve their performance. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{docs/fig/mnist_cmp_cnn_pf.png}
    \vspace{-0.1in}
    \caption{Combining WF-DP with PrivateFL (PFL). Note that $\epsilon=6.76/3.38/1.69$ represents $\sigma=0.05/0.1/0.2$.}
    \label{fig:femnist}
    \vspace{-0.2in}
\end{figure}

==> docs/old/solution_old.tex <==
\vspace{-0.05in}
\section{Practical Mechanism for achieving \texorpdfstring{$(\epsilon,\delta)$}{(e,d)}-DP}
\label{sec:solution}
\subsection{Overview}
In this section, we introduce a novel mechanism called Water-Filling DP (WF-DP) to achieve $(\epsilon,\delta)$-DP in FL with SA, without relying on any assumptions about the singularity of covariance matrix of gradient noise. The key novelty of WF-DP is that it leverages the inherent noise contained in the aggregated model updates from other non-sensitive users to reduce the amount of additional noise required for ensuring DP (or even to entirely avoid adding additional noise in non-singular covariance matrix scenarios). 

As discussed in Section \ref{sec:theory}, there are two issues that may make the aggregated model update from other users fail to provide DP guarantee: 1) its covariance matrix is singular, which is common in real-world popular deep neural network models due to over-parameterization \cite{du2018gradient, allen2019convergence} (see Section \ref{subsec:gaussian_singular}); and 2) the gradient noise does not follow a Gaussian distribution (see Section \ref{subsec:non_guassian}). WF-DP addresses the first issue by lifting the zero eigenvalues (and some small eigenvalues) in the covariance matrix of each user's model update, in order to guarantee their non-singularity. To solve the second issue, WF-DP uses Gaussian gradient sampling noise (see Assumption \ref{assum2}), together with the revised non-singular covariance matrix. We describe the details of WF-DP in the rest of this section. 
%\jiang{Note that we only apply WF-DP for non-sensitive users.}


% \begin{algorithm}
% \caption{WF-DP algorithm}
% \begin{algorithmic}[1]
% \State \textbf{Input:} $D_i$, $\theta^{(t)}$, $\mathbb{U}_{s}$, $\mathbb{U}_{ns}$, $C$, $B$, $q$, $M$, $\epsilon$, and $\delta$.
% \State \textbf{Output:} A Gaussian model update $x_{i}^{(t)}$
% \State Calculated the minimum eigenvalue $\sigma^2$ from Eq. (\ref{eq:wfdp}).
% \If {Use FedSGD protocol}
% \State Calculate a gradient update for each data point in $D_i$ (get $|D_i|$ gradient updates in total).
% \If {$i\in\mathbb{U}_{s}$}
% \State Clip each gradient update to bound its $L_2$-norm by $C$.
% \ElsIf {$i\in\mathbb{U}_{ns}$}
% \State Estimate the mean and covariance matrix of these $|D_i|$ gradient updates as $\mu_i^{(t)}$ and $\Sigma_{i,single}^{(t)}$.
% \State Calculate the estimated covariance matrix of model update as $\Sigma_i^{(t)}=\frac{\Sigma_{i,single}^{(t)}}{B}$.
% \EndIf
% \ElsIf{Use FedAvg protocol}
% \For {$m$ in $1,...,M$}
% \State Initialize the local model with $\theta^{(t-1)}$
% \State Randomly shuffle $D_i$.
% \State Use FedAvg to calculate the local model update $x_{i,m}^{(t)}$. 
% \If {$i\in\mathbb{U}_{s}$}
% \State Clip $x_{i,m}^{(t)}$ to bound its $L_2$ norm by $C$.
% \EndIf
% \EndFor
% \If {$i\in\mathbb{U}_{ns}$}
% \State Estimate the mean and covariance matrix of these $M$ local model updates as $\mu_i^{(t)}$ and $\Sigma_{i}^{(t)}$.
% \EndIf
% \EndIf
% \If {$i\in\mathbb{U}_{s}$}
% \State Run SVD on $\Sigma_i^{(t)}$ as $\Sigma_i^{(t)}=U_i^{(t)}\Lambda_i^{(t)}(U_i^{(t)})^{(t)}$.
% \For {the $i$-th eigenvalue $\lambda_i^{(t)}$ in $\Lambda_i^{(t)}$}
% \If {$\lambda_i^{(t)} < \sigma^2$}
% \State $\lambda_i^{(t)} \gets \sigma^2$
% \EndIf
% \EndFor
% \State Denote the updated $\Lambda_i^{(t)}$ as $\Lambda_{i,new}^{(t)}$ and calculate the new covariance matrix as $\Sigma_{i,new}^{(t)}=U_i^{(t)}\Lambda_{i,new}^{(t)}(U_i^{(t)})^{T}$.
% \State Sample a Gaussian gradient with mean $\mu_i^{(t)}$ and covariance matrix $\Sigma_{i,new}^{(t)}$.
% \ElsIf {$i\in\mathbb{U}_{ns}$}

% \EndIf
% \end{algorithmic}
% \label{algo1}
% \end{algorithm}

\vspace{-0.08in}
\subsection{Algorithm design}
%In this subsection, we describe the details of WF-DP algorithm for both FedSGD and FedAvg protocol, where the input parameters 
The input of the WF-DP algorithm for each user $i$ includes the local dataset $D_i$, the current global model parameters $\theta^{(t)}$, the number of users $N$ participating in FL, the clip value $C$, mini-batch size $B$, sampling time $M$, the lower bound for minimal eigenvalue budget $\sigma^2$, and the relaxation item $\delta$. Note that without loss of generality, we assume that the input parameters are the same across users.

% \noindent\textbf{Set privacy budget.} First, we calculate the minimum noise level  $\sigma^2$ required to achieve a target $(\epsilon^{(t)},\delta)$-DP guarantee, using the following equation:
% \begin{equation}
% \label{eq:wfdp}
%     \sigma^2=\frac{C_0}{N\epsilon^{(t)}}
% \end{equation}
% where $C_0 = ... $.
% Once the $\sigma$ is set, WF-DP will guarantee DP with the following $\epsilon^{(t)}$ value:
First, user $i$ will use its local dataset $D_i$ to calculate the mean gradient and covariance matrix of gradient noise as $\mu_i^{(t)}$ and $\Sigma_{i}^{(t)}$ respectively. We describe this process for FedSGD and FedAvg separately below.

\noindent\textbf{Calculate covariance matrix in FedSGD.} In FedSGD, for each local training data points, user $i$ will calculate a gradient from this data point and clip its $L_2$ norm to make it upper bounded by constant $C$. 
After obtaining $|D_i|=D$ clipped gradient vectors, user $i$ uses them to calculate the mean $\mu_i^{(t)}=\frac{1}{D}\sum_{j=1}^{D}g_{i,j}^{(t)}$ and covariance matrix $\Sigma_{i}^{(t)}=\frac{1}{BD}\sum_{j=1}^{D}g_{i,j}^{(t)}(g_{i,j}^{(t)})^T$. 
%Since the final model update in FedSGD is the average of $B$ individual gradients sampled in an i.i.d fashion (see Eq. (\ref{eq:fedsgd1})), its covariance matrix will be $\Sigma_{i}^{(t)}=\frac{\Sigma_{i,single}^{(t)}}{B}$.

\noindent\textbf{Estimate covariance matrix in FedAvg.} In FedAvg, each user generates $M$ local model update samples to estimate its covariance matrix. To generate the $m$-th sample, user $i$ first needs to initialize its local model with $\theta^{(t-1)}$. Then, user $i$ needs to randomly shuffle its local dataset $D_i$, and then run FedAvg to calculate the local model update as $x_{i,j}^{(t)}$. Once user $i$ collects $D$ model update samples, it will estimate their mean and covariance matrix as $\mu_{i}^{(t)}=\frac{1}{D}\sum_{j=1}^{D}x_{i,j}^{(t)}$ and $\Sigma_{i}^{(t)}=\frac{1}{BD}\sum_{j=1}^{D}x_{i,j}^{(t)}(x_{i,j}^{(t)})^T$ respectively.

\noindent\textbf{Run SVD and lower bound the smallest eigenvalue.} Next, user $i$ will run SVD on its estimate covariance matrix as $\Sigma_i^{(t)}=U_i^{(t)}\Lambda_i^{(t)}(U_i^{(t)})^{T}$, and clip the eigenvalues in $\Lambda_i^{(t)}$ such that all eigenvalues are lower bounded by $\sigma^2$. Define the updated diagonal matrix with bounded eigenvalues as $\Lambda_{i,+}^{(t)}$. The revised covariance matrix can be calculated as $\Sigma_{i,+}^{(t)}=U_i^{(t)}\Lambda_{i,+}^{(t)}(U_i^{(t)})^{T}$. Note that to make the SVD process efficient, we split the $d$-dimension gradient into $k$ parts, estimate the covariance matrix for each part, run SVD on these $k$ covariance matrices separately, and concatenate them into the final covariance matrix. By running SVD approximately, the time complexity of SVD will be reduced from $O(d^3)$ to $O(k\frac{d}{k}^3)=O(\frac{d^3}{k^2})$ (see similar approaches in \cite{liu2014additive, delattre2012blockwise,tamilmathi2022tensor}), without affecting the $\epsilon$ bound we have.

\noindent\textbf{Generate Gaussian model update.} Finally, each user samples a Gaussian model update with mean $\mu_i^{(t)}$ and covariance matrix $\Sigma_{i,new}^{(t)}$ (see Eq. (\ref{eq:gaussin_gradient}).



\begin{thm} [DP guarantees of WF-DP algorithm]
\label{theorem_wf}
Given the input parameters of WF-DP, for any $\alpha\in(1,\frac{N\sigma^2D}{2C^2})$, the aggregated model update using WF-DP can provide $(\alpha,\epsilon^{(t)})$-RDP and $(\epsilon^{(t)}+\frac{\log(1/\delta)}{\alpha-1},\delta)$-DP guarantees to any user $i$'s local dataset, where the $\epsilon^{(t)}$ of each training round is given as follows:
\begin{equation}
\label{eq:wfdp}
\epsilon^{(t)} =
    (\frac{2\alpha BC^2}{D^2}+\frac{2\alpha C^2}{(\alpha-1)D})\frac{1}{N\sigma^2-\frac{2\alpha C^2}{D}}.
\end{equation}
\end{thm}
\begin{proof}
We define the change of covariance matrix after applying WF-DP as: 
\begin{equation}
    \Sigma_{i,\Delta}^{(t)} = \Sigma_{i,+}^{(t)} - \Sigma_{i}^{(t)}.
\end{equation}
Since WF-DP only increases the eigenvalues of the original covariance matrix by maximally $\sigma^2$,   $\Sigma_{i,\Delta}^{(t)}$ will be semi-definite with maximal eigenvalue upper bounded by $\sigma^2$. Then, consider $\Sigma_{i,+}^{(t),1}$ and $\Sigma_{i,+}^{(t),2}$, which are two instances of $\Sigma_{i,+}^{(t)}$ by changing one data point in $D_i$, we have:
\begin{equation}
\begin{aligned}
      \Sigma_{i,+}^{(t),2}-\Sigma_{i,+}^{(t),1}=&\frac{1}{BD}(g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T-g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T) + \Delta\Sigma_{i,\Delta}^{(t)},  
\end{aligned}
\end{equation}
where $\Delta\Sigma_{i,\Delta}^{(t)} = \Sigma_{i,\Delta}^{(t),2}-\Sigma_{i,\Delta}^{(t),1}$. 

Since removing $g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T$ decreases the eigenvalues, which may cause some eigenvalues below smaller than $\sigma^2$, WF-DP needs to refill eigenvalues smaller than $\sigma^2$. Hence, we have $\Delta\Sigma_{i,\Delta}^{(t)}\preceq \frac{1}{BD}g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T$. This says, by changing one data point in user $i$'s local dataset, WF-DP will at most increase $\Sigma_{i,+}^{(t),1}$ by $\frac{1}{BD}g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T$ to refill small eigenvalues. 
Moreover, since adding $g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T$ increases the eigenvalues, WF-DP may lift eigenvalues smaller than $\sigma^2$ less. Hence, we have $\Delta\Sigma_{i,\Delta}^{(t)}\succeq -\frac{1}{BD}g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T$. This says, by changing one data point in user $i$'s local dataset, WF-DP will at most reduce $\Sigma_{i,+}^{(t),1}$ by $\frac{1}{BD}g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T$. Formally, we have:
\begin{equation}
\begin{aligned}
      -\frac{1}{BD}g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T \preceq \Delta\Sigma_{i,\Delta}^{(t)} \preceq \frac{1}{BD}g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T
\end{aligned}
\end{equation}

Since $||g_{i,1}^{(t),l}||_2\leq C$, we can derive that $\forall~x\in\mathbf{R}^K$,
\begin{equation}
\begin{aligned}
      &x^T(\Sigma_{i,+}^{(t),2}-\Sigma_{i,+}^{(t),1})x\\
      \geq &-x^T(\frac{1}{BD}g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T+\frac{1}{BD}g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T)x\geq -\frac{2C^2}{BD}x^Tx.  
\end{aligned}
\end{equation}
Therefore, $\forall~x\in\mathbf{R}^K$, 
\begin{equation}
\begin{aligned}
&x^T\Sigma_{\alpha,+} x=x^T((1-\alpha)\Sigma_{1,+} + \alpha\Sigma_{2,+})x \\
=&x^T\Sigma_1 x + x^T\frac{\alpha}{B}(\Sigma_{i,+}^{(t),2}-\Sigma_{i,+}^{(t),1})x\\
\geq & (\frac{N\sigma^2}{B}-\frac{2\alpha C^2}{BD})x^Tx.
\end{aligned}
\end{equation}
Moreover, we can derive
\begin{equation}
\Sigma_{2,+}\preceq \Sigma_{1,+} + \frac{1}{BD}g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T +  \frac{1}{BD}g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T,
\end{equation}
and 
\begin{equation}
\Sigma_{1,+}\preceq \Sigma_{\alpha,+} + \frac{\alpha}{BD}g_{i,1}^{(t),2}(g_{i,1}^{(t),2})^T +  \frac{\alpha}{BD}g_{i,1}^{(t),1}(g_{i,1}^{(t),1})^T.
\end{equation}
Following the proof of Theorem \ref{theorem1}, we derive:
\begin{equation}
\label{eq:rd_bound_3}
\begin{aligned}
&D_{\alpha}(\mathcal{M}_{\{D_i^1\cup D_{-i},\theta^{(t)}\}} \| \mathcal{M}_{\{D_i^2\cup D_{-i},\theta^{(t)}\}}) \\
\leq & \frac{\alpha}{2}(\Delta \bar g_{i}^{(t)})^T \Sigma_{\alpha,+}^{-1}\Delta \bar g_{i}^{(t)}-\frac{1}{2(\alpha - 1)}\ln\frac{|\Sigma_{\alpha,+}|}{|\Sigma_{1,+}|^{1-\alpha}|\Sigma_{2,+}|^{\alpha}}.\\
\leq & \frac{2\alpha C^2}{D^2}\frac{1}{\frac{N\sigma^2}{B}-\frac{2\alpha C^2}{BD}} + \frac{\alpha C^2}{(\alpha-1)BD}(\frac{1}{\frac{N\sigma^2}{B}}+\frac{1}{\frac{N\sigma^2}{B}-\frac{2\alpha C^2}{BD}})\\
= & (\frac{2\alpha BC^2}{D^2}+\frac{2\alpha C^2}{(\alpha-1)D})\frac{1}{N\sigma^2-\frac{2\alpha C^2}{D}}=\epsilon^{(t)}.
\end{aligned}
\end{equation}
Hence, the aggregated model update using WF-DP can provide $(\alpha,\epsilon^{(t)})$-RDP and $(\epsilon^{(t)}+\frac{\log(1/\delta)}{\alpha-1},\delta)$-DP guarantees to any user $i$'s local dataset.
\end{proof}
    
\noindent\textbf{Accumulative privacy loss.} So far, we analyze the $\epsilon^{(t)}$ value for each training round. Since we have $T$ training rounds in total,the $\epsilon$ across all $T$ training rounds will increase with $T$. According to the simple composition theorem in DP \cite{dwork2014algorithmic}, $\epsilon$ for $T$ training round will be upper bounded by $\epsilon^{(t)}T$. However, recent works such as \cite{abadi2016deep,gopi2021numerical} have demonstrated that the optimal upper bound for $T$ can be $O(q\epsilon^{(t)}\sqrt{T})$, where $q$ is the data or user sampling ratio during training round. To numerically estimate the accumulate $\epsilon$ across $T$ training round, we use the algorithm proposed in \cite{gopi2021numerical}, which can take as input the noise level $\sigma$, the sampling ratio $q$ and the total training round $T$, and then output the estimated $\epsilon$ value at the end of training. Note that in FedSGD, $q=\frac{B}{|D_i|}$ is the sampling ratio of mini-batch size.  In FedAvg, since we use all the local dataset for calculating the local model updates, we can not amplify DP via data samping. Instead, we can amplify DP via user selection (i.e. randomly select a subset of users in each training round, see \cite{zhang2022understanding}). 

\subsection{Discussion about WF-DP}
\label{subsec:intuitive_cmp}
\noindent\textbf{Type of DP guarantee in WF-DP.} WF-DP can be used in both FedSGD and FedAvg protocol to provide DP. Specifically, in FedSGD protocol where each user samples a data batch to calculate the model update, WF-DP provides sample-level DP guarantee for sensitive users, which means that the server cannot identify the change of one data point in a sensitive user's local dataset by observing the aggregated model updates. In FedAvg protocol where each user uses their whole dataset to calculate the model update, WF-DP provides client-level DP that is stronger than sample-level privacy, which means that the server cannot identify the participation of one user by observing the aggregated model updates. 

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.85\textwidth]{docs/fig/sys_fig_1.pdf}
    \caption{Noise added by WF-DP.}
    \label{fig:wf_dp}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.48\linewidth}
    \includegraphics[width=0.85\textwidth]{docs/fig/sys_fig_2.pdf}
    \caption{Noise added by DDP.}
    \label{fig:ldp}
  \end{subfigure}
  \vspace{-0.1in}
  \caption{Comparison of the amount of noise added by WF-DP and DDP.}
  \label{fig:noise_dp}
  \vspace{-0.2in}
\end{figure}

\noindent\textbf{Intuitive comparison of WF-DP with DDP}
Figure \ref{fig:noise_dp} compares the amount of noise added by WF-DP and DDP, where the $x$-axis represents the index of each eigenvalue and the $y$-axis represents the value of each eigenvalue. The noise contained in the aggregated model update is randomly distributed in the directions of all eigenvectors, and each eigenvalue measures the variance of the noise in each eigenvector direction. When the eigenvalue is larger than $\sigma^2$ (i.e. the amount of noise we need for achieving our privacy target), then the aggregated model update can already provide enough privacy protection, without needing additional noise. Since WF-DP leverages the noise contained in the aggregated model update, by only adding noise to the eigenvector directions where the eigenvalues are smaller than  $\sigma^2$, it can add less noise compared with DDP, as shown in Figure \ref{fig:wf_dp} and \ref{fig:ldp}. Hence, for the same level of privacy, WF-DP can lead to higher model accuracy.




% Note that we use block-wise SVD in order to run SVD efficiently. We use Gaussian gradient descent since we can explicitly calculate the $\epsilon$ and $\delta$ for DP guarantee. Moreover, prior work \cite{wu2020noisy} has demonstrated that Gaussian gradient descent can achieve comparable performance with SGD in terms of both model accuracy and converge rate.




==> docs/old/theory_old.tex <==
\section{Main Theoretical Results}
\label{sec:theory}
In this section, we analyze under what conditions FL with SA can provide DP guarantee when using FedSGD protocol. Note that while our theorems are derived using FedSGD protocol, they can be generalized for FedAvg protocol (see Remark 2).


\subsection{Basic assumptions}
We start by making the following assumption about FedSGD protocol in our analysis, which has been widely used in FL \cite{kairouz2019advances}.

\begin{assump}[User types] Assume that users are divided into two types: 1) sensitive users which desire worst-case privacy guarantees and hence clip their model updates; 2) non-sensitive users which do not desire worst-case privacy guarantees and hence do not clip their model updates. 
%For sensitive users, we assume that they use sensitive data during FL and need their model updates being protected. For non-sensitive users, we assume that they do not use sensitive data during FL and thus do not need their model updates being protected. 
We define the set of sensitive users as $\mathbb{U}_s$ and the set of non-sensitive users as $\mathbb{U}_{ns}$ respectively.
\label{assum0}
\end{assump}


\begin{assump}[IID sampling with replacement and clipping for sensitive users]  Assume that each sensitive user $i$  uniformly and randomly samples $B$ data points with replacement from its local dataset $D_{i}$ as a mini-batch $\mathcal{B}_{i}^{(t)}$ with size $B$ at step $t$ 
%with sampling ratio $q_{i}^{(t)}=\frac{B}{|D_{i}|}$, 
to compute the model update. Moreover, assume that sensitive users will clip their model updates. Formally, the model update of sensitive user $i$ is computed as follows:
\begin{equation}
\label{eq:fedsgd1}
x_{i}^{(t)} = \frac{1}{B} \sum_{b \in \mathcal{B}_{s,i}^{(t)} } g_{i}( \theta^{(t)}, b) =  \frac{1}{B} \sum_{b \in \mathcal{B}_{s,i}^{(t)} }clip(\frac{\partial L(\theta^{(t)},b)}{\partial \theta^{(t)}}, C),
\end{equation}
% and
% \begin{equation}
% \label{eq:fedsgd2}
% g_{i}(\theta^{(t)}, b) =
% \begin{cases}
%     clip(\frac{\partial L(\theta^{(t)},b)}{\partial \theta^{(t)}}, C), & \text{if $i\in\mathbb{U}_{s}$} \\ 
%     \frac{\partial L(\theta^{(t)},b)}{\partial \theta^{(t)}},  & \text{if $i\in\mathbb{U}_{ns}$}
% \end{cases}
% \end{equation}
where $clip(x,C)=\frac{Cx}{max(||x||_2,C)}$ is a clipping function to bound the norm of vector $x$ by constant $C$. Then, each individual model update $g_i( \theta^{(t)}, b)\in\mathrm{R}^d$ can be viewed as a random vector. Assume that it has mean $\mu_i^{(t)}$ and covariance matrix $\Sigma_{i,single}^{(t)}$. Due to IID sampling, the model update $x_i^{(t)}$ will be a random vector with mean $\mu_i^{(t)}$ and covariance matrix 
 $\Sigma_i^{(t)}=\frac{\Sigma_{i,single}^{(t)}}{B}$.
\label{assum1}
\end{assump}

Moreover, we define the aggregated model update from all non-sensitive users at step $t$ as $x_{ns}^{(t)}=\sum_{i\in\mathbb{U}_{ns}}x_{i}^{(t)}$, which is a random vector with mean $\mu_{ns}^{(t)}=\sum_{i\in\mathbb{U}_{ns}}\mu_i^{(t)}$ and covariance matrix $\Sigma_{ns}^{(t)}=\sum_{i\in\mathbb{U}_{ns}}\Sigma_i^{(t)}$. 


\noindent\textbf{Necessity of Assumptions \ref{assum0} and \ref{assum1}.} In the above two assumptions, we assume there is a set of sensitive users who will clip their model updates and another set of non-sensitive users who do not clip their model updates. This is necessary for achieving DP guarantee with existing DP mechanisms which needs bounded sensitivity of local data and unbounded noise (e.g. Guassian mechanisms, Laplace mechanism, Exponential mechanism \cite{dwork2014algorithmic}). Specifically, without clipping the model update, the sensitivity of a user's model update by varying one data point in their local dataset will be unbounded. In this case, DP can not be guaranteed. On the other hand, if a user clips her/his model update, then this model update will be bounded and thus cannot be used as unbounded noise with respect to other users to provide DP guarantee in FL. Therefore, a user who needs DP protection can not offer DP protection for other users. In other words, if all users are sensitive users, DP can not be guaranteed in FL with SA based on the analysis framework of DP mechanism with unbounded noise. While there are a few recent works studying DP mechanisms with bounded noise 
%\cite{liu2018generalized} - prob. DP...
\cite{holohan2018bounded,dagan2022bounded}, in this paper we consider traditional DP mechanisms that require unbounded noise and leave the question of whether DP mechanisms with bounded noise may be applied to our setup as future work.
\footnote{Recently, \cite{dagan2022bounded} proposed a truncated Laplacian mechanism that may guarantee ($\epsilon$, $\delta$) DP. One challenge if we were to apply this mechanism in our context is that prior work has demonstrated that model updates can be close to Gaussian and we use this in our analysis, see end of Section \ref{sec:theory}, whereas there isn't similar prior art evidence that model updates can be close to a truncated Laplacian distribution.}


\subsection{Gaussian model update with non-singular covariance matrix}
\label{subsec:gaussian_non_singular}
We first consider the case where the model update of each non-sensitive user in $\mathbb{U}_{ns}$ is a Gaussian random vector with non-singular covariance matrix, to present our first theorem. This is motivated by the following two reasons: 1) A variety of prior works on investigating the behavior of SGD have assumed that the stochastic noise in the model update follows a multivariate Gaussian distribution (e.g. \cite{shang2015covariance,zhu2018anisotropic, mandt2017stochastic}), and 2) a closed-form $\epsilon$ bound in DP can be derived for Gaussian noise. Formally, we make the following assumption:

\begin{assump}[Gaussian model update with non-singular covariance matrix for non-sensitive users] Assume that at step $t$, for any non-sensitive user $i\in\mathbb{U}_{ns}$, its model update $x_{i}^{(t)}$ is a Gaussian random vector, with mean $\mu_i^{(t)}$, non-singular covariance matrix $\Sigma_i^{(t)}$ and the smallest eigenvalue of $\Sigma_{i}^{(t)}$ is $\lambda_{i,min}^{(t)}$.
\label{assum2}
\end{assump}
Based on Assumption \ref{assum2}, we can derive that the aggregated model update from all non-sensitive users 
$x_{ns}^{(t)}=\sum_{j\in\mathbb{U}_{ns}}x_{j}^{(t)}$ will be Gaussian, with non-singular covariance matrix $\Sigma_{ns}^{(t)}=\sum_{j\in\mathbb{U}_{ns}}\Sigma_{j}^{(t)}$. We define the smallest eigenvalue of $\Sigma_{ns}^{(t)}$ as $\lambda_{min}^{(t)}$, which can be bounded as follows:
\begin{equation}
\label{eq:eigen_bound}
    \lambda_{min}^{(t)}\geq\sum_{j\in\mathbb{U}_{ns}}\lambda_{j,min}^{(t)}.
\end{equation}

With the above definitions and assumptions, we can now
state and prove our first theorem below.
\begin{thm}
Under Assumption \ref{assum0},\ref{assum1},\ref{assum2}, the aggregated model update from any non-sensitive users $x_{ns}^{(t)}$ at step $t$ can provide $(\epsilon_i^{(t)},\delta)$-DP for any sensitive user $i$'s model update ($i\in\mathbb{U}_{s}$), where $\epsilon_i^{(t)}=p(\lambda_{min}^{(t)}, \delta)$,
%\frac{8C^2\log\frac{1.25}{\delta}}{\epsilon^2}$}

\begin{equation}
\label{eq:lambda1}
p(\lambda_{min}^{(t)}, \delta) =
\begin{cases}
    \frac{2C\sqrt{2\log\frac{1.25}{\delta}}}{B\sqrt{\lambda_{min}^{(t)}}},& \text{$\lambda_{min}^{(t)} >\lambda_0,\delta \in(0,1)$} \\ 
    max(1,\frac{2C^2}{B^2\lambda_{min}^{(t)}}), & \text{$\lambda_{min}^{(t)} \in(0, \lambda_0],\delta \in(0,f(\epsilon_{i}^{(t)}))$},
\end{cases}
\end{equation}
$f(\epsilon_{i}^{(t)}) = \frac{1}{2}-\frac{e^{-3\epsilon_i^{(t)}}}{\sqrt{4\pi\epsilon_i^{(t)}}}$, and $\lambda_0=\frac{4C^2\sqrt{2\log\frac{1.25}{\delta}}}{B^2}$

% where $\epsilon_i^{(t)}\leq\frac{2C\sqrt{2\log\frac{1.25}{\delta}}}{\sqrt{\lambda_{min}^{(t)}}}\leq\frac{2C\sqrt{2\log\frac{1.25}{\delta}}}{\sqrt{\sum_{j\in\mathbb{U}_{ns}}\lambda_{j,min}^{(t)}}}$.
\label{theorem1}
\end{thm}

\begin{proof}
From Assumption \ref{assum2}, we know that the aggregated model update from non-sensitive users $x_{ns}$ is a Gaussian random vector with non-singular covariance matrix $\Sigma_{ns}^{(t)}$. Hence, we can perform the singular value decomposition on $\Sigma_{ns}^{(t)}$ as follows:
\begin{equation}
\Sigma_{ns}^{(t)}=U_{ns}^{(t)}\Lambda_{ns}^{(t)}(U_{ns}^{(t)})^{T}=U_{ns}^{(t)}(\Lambda_{ns}^{(t)})^{\frac{1}{2}}(\Lambda_{ns}^{(t)})^{\frac{1}{2}}(U_{ns}^{(t)})^{T}.
\end{equation}
Define $L_{ns}^{(t)}=U_{ns}^{(t)}(\Lambda_{ns}^{(t)})^{\frac{1}{2}}$, which has full rank. Then we have $\Sigma_{ns}^{(t)}=L_{ns}^{(t)}(L_{ns}^{(t)})^{T}$. Since the smallest eigenvalue of $\Sigma_{ns}^{(t)}$ is $\lambda_{min}^{(t)}$, the smallest eigenvalue of $L_{ns}^{(t)}$ is $\sqrt{\lambda_{min}^{(t)}}>0$. 

Assume that $x_{i,1}^{(t)}$ and $x_{i,2}^{(t)}$ are two model update instances of $x_{i}^{(t)}$ at step $t$, which are calculated from two local datasets $D_i^{1}$ and $D_i^{2}$ differing by only one data point. Then, $\forall X \subseteq Range(x_{i}^{(t)}+x_{ns}^{(t)})$ and $\forall$ $x_{i,1}^{(t)}$ and $x_{i,2}^{(t)}$,  we have:
\begin{align}
    \frac{Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]}{Pr[x_{i,2}^{(t)}+x_{ns}^{(t)}\in X]}
    =&\frac{Pr[(L_{ns}^{(t)})^{-1}(x_{i,1}^{(t)}+x_{ns}^{(t)}-\mu_{ns}^{(t)})\in Y]}{Pr[(L_{ns}^{(t)})^{-1}(x_{i,2}^{(t)}+x_{ns}^{(t)}-\mu_{ns}^{(t)})\in Y]}\\
    =&\frac{Pr[n_{i,1}^{(t)}+n_{ns}^{(t)}\in Y]}{Pr[n_{i,2}^{(t)}+n_{ns}^{(t)}\in Y]}
\end{align}
where we define $n_{i,1}^{(t)}=(L_{ns}^{(t)})^{-1}x_{i,1}^{(t)}$, $n_{i,2}^{(t)}=(L_{ns}^{(t)})^{-1}x_{i,2}^{(t)}$, $n_{ns}^{(t)}=(L_{ns}^{(t)})^{-1}(x_{ns}^{(t)}-\mu_{ns}^{(t)})$, and $Y=\{(L_{ns}^{(t)})^{-1}(x-\mu_{ns}^{(t)}) | x\in X\}$. 

Since $x_{ns}^{(t)}\sim \mathcal{N}(\mu_{ns}^{(t)}, L_{ns}^{(t)}(L_{ns}^{(t)})^{T})$, we have $n_{ns}^{(t)}\sim \mathcal{N}(0,I_d)$, where $I_d$ is an identity matrix with $d$ dimensions and hence $n_{ns}^{(t)}$ can be viewed as the noise vector used in standard Gaussian mechanism. Moreover, we have:
\begin{align}
\label{eq:delta}
    \Delta&=\max_{\forall x_{i,1}^{(t)}, x_{i,2}^{(t)}}||n_{i,1}^{(t)}-n_{i,2}^{(t)}||_2=\max_{\forall x_{i,1}^{(t)}, x_{i,2}^{(t)}}||(L_{ns}^{(t)})^{-1}(x_{i,1}^{(t)}-x_{i,2}^{(t)})||_2\\
    &\leq\frac{2C}{B\sqrt{\lambda_{min}^{(t)}}} \leq\frac{2C}{B\sqrt{\sum_{j\in\mathbb{U}_{ns}}\lambda_{j,min}^{(t)}}}
\end{align} 
Based on Eq. (\ref{eq:lambda1}), in high privacy region where $\epsilon_i^{(t)}\in(0,1)$ and $\delta \in(0,1)$,
we have $\frac{\Delta\sqrt{2\log\frac{1.25}{\delta}}}{\epsilon_i^{(t)}}\leq1$. In low privacy region where $\epsilon_i^{(t)}\in[1,+\infty)$ and $\delta \in(0,\frac{1}{2}-\frac{e^{-3\epsilon_i^{(t)}}}{\sqrt{4\pi\epsilon_i^{(t)}}})$, we have $\frac{\Delta}{\sqrt{2\epsilon_i^{(t)}}}\leq1$. 
Therefore, according to the standard analytic results on Gaussian DP mechanism in \cite{dwork2014algorithmic,balle2018improving}, for both high privacy region (i.e. $\epsilon_i^{(t)}\in(0,1)$) and low privacy region (i.e. $\epsilon_i^{(t)}\geq 1$), we have:
\begin{align}
    Pr[n_{i,1}^{(t)}+n_{ns}^{(t)}\in Y]\leq e^{\epsilon_i^{(t)}}{Pr[n_{i,2}^{(t)}+n_{ns}^{(t)}\in Y]} + \delta,
\end{align} and hence:
\begin{align}
    Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]
    \leq e^{\epsilon_i^{(t)}}{Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]} + \delta.
\end{align}
\end{proof}
\vspace{-.05in}

\begin{corollary} (IID non-sensitive users with non-singlular covariance matrix) 
\label{coro1}
Under Assumption \ref{assum0}, \ref{assum1}, \ref{assum2}, we further assume that all non-sensitive users’ local datasets are randomly sampled IID from a common distribution, which implies that the gradient updates of all non-sensitive users come from the identical distribution with the same mean $\mu^{(t)}$ and covariance matrix $\Sigma^{(t)}$ (i.e., $\forall j\in\mathbb{U}_{ns}, x_j^{(t)}\sim \mathcal{N}(\mu^{(t)}, \Sigma^{(t)})$). Let $\lambda_{0,min}^{(t)}$ be the smallest eigenvalue of $\Sigma^{(t)}$. Then, the aggregated gradient from other users $x_{ns}^{(t)}$ at step $t$ can provide $(\epsilon_i^{(t)},\delta)$-DP for sensitive user $i\in\mathbb{U}_{s}$ with $\epsilon_i^{(t)}=\frac{2C\sqrt{2\log\frac{1.25}{\delta}}}{B\sqrt{|\mathbb{U}_{ns}|\lambda_{min}^{(t)}}}$ for high privacy region ($\epsilon_i^{(t)}\in(0,1)$) and $\epsilon_i^{(t)}=\frac{2C^2}{B^2|\mathbb{U}_{ns}|\lambda_{0,min}^{(t)}}$ for low privacy region ($\epsilon_i^{(t)}\geq 1$),
where $|\mathbb{U}_{ns}|$ is the number of non-sensitive users.
\end{corollary}

\begin{proof}
\label{proof_coro1}
See Appendix \ref{sec:proof_coro1} for details.
    % \jiang{Since $\forall j\in\mathbb{U}_{ns}, x_j^{(t)}\sim \mathcal{N}(\mu^{(t)}, \Sigma^{(t)})$, we have $\Sigma_{ns}^{(t)}=\sum_{j\in\mathbb{U}_{ns}}\Sigma_{j}^{(t)}=|\mathbb{U}_{ns}|\Sigma^{(t)}$. Hence, the smallest eigenvalue of $\Sigma_{ns}^{(t)}$ will be $|\mathbb{U}_{ns}|\lambda_{0,min}^{(t)}$. Based on Eq. \ref{eq:lambda1} in Theorem \ref{theorem1}, in high privacy region where $\epsilon_i^{(t)}\in(0,1)$, we have $\epsilon_i^{(t)}=\frac{2C\sqrt{2\log\frac{1.25}{\delta}}}{B\sqrt{|\mathbb{U}_{ns}|\lambda_{0,min}^{(t)}}}$. In low privacy region where $\epsilon_i^{(t)}\geq 1$, we have $\epsilon_i^{(t)}=\frac{2C^2}{B^2|\mathbb{U}_{ns}|\lambda_{0,min}^{(t)}}$.}
\end{proof}
\vspace{-.05in}

Both Theorem \ref{theorem1} and and Corollary \ref{coro1} indicate that the $\epsilon$ for sensitive users in FL with SA depends on two main factors: 1) the number of non-sensitive users participating in FL with SA; 2) the minimal eigenvalues of the model update covariance matrix from non-sensitive users. Specifically, as we increase the number of non-sensitive users $|\mathbb{U}_{ns}|$, the $\epsilon$ will decay, where the decay rate will be $\frac{1}{\sqrt{|\mathbb{U}_{ns}|}}$ for IID users in high privacy region and $\frac{1}{|\mathbb{U}_{ns}|}$ for IID users in low privacy region. Moreover, when $\lambda_{j,min}^{(t)} ( j\in\mathbb{U}_{ns}$), i.e., the minimal eigenvalues of other non-sensitive users' covariance matrix increase, $\epsilon$ for sensitive users will also decrease.

However, it is worth noting that both Theorem \ref{theorem1} and and Corollary \ref{coro1} rely on the non-singular covariance matrix assumption (i.e. Assumption \ref{assum2}), which may not easily hold in practice. Especially in applications using deep neural networks, the number of training data points is typically smaller than the number of model parameters (i.e. over-parameterization), and as a result the covariance matrix of the model update will be singular \cite{du2018gradient, allen2019convergence}. 

Motivated by this, we next consider the case where the aggregated model update of each user is a Gaussian random vector with singular covariance matrix.

\vspace{-0.05in}
\subsection{Gaussian model update with singular covariance matrix}
\label{subsec:gaussian_singular}
Before presenting our second theorem, we formally make the following assumptions:
\begin{assump}[Singular covariance matrix for non-sensitive users] Assume that at step $t$, for any non-sensitive users user $j\in\mathbb{U}_{ns}$, its model update $x_{j}^{(t)}$ has a singular covariance matrix $\Sigma_j^{(t)}$. Moreover, suppose running SVD on $\Sigma_{j}^{(t)}$ will derive $\Sigma_{j}^{(t)}=V_{j}^{(t)}\Lambda_j^{(t)}(V_{j}^{(t)})^{T}$, where $V_{j}^{(t)}=[v_{j,1},...,v_{j,k_j}]$, $\Lambda_j^{(t)}=diag(\lambda_{j,1},...,\lambda_{j,k_j})$ is a diagonal matrix with non-zero eigenvalues in its diagonal axis and zeros in other places, and $k_j$ is the number of non-zero eigenvalues of $\Sigma_{j}^{(t)}$. 
\label{assum3}
\end{assump}
For non-sensitive user $j$, when $x_{j}^{(t)}$ is a Gaussian random vector and Assumption \ref{assum3} holds, we can rewrite $x_j^{(t)}$ as $x_j^{(t)}=\mu_j^{(t)} + V_{j}^{(t)}\Lambda_j^{(t),\frac{1}{2}}n_j^{(t)}$, where $n_j^{(t)}\sim N(0,I_{k_j})$ is a standard normal random vector. We define $span(V_{j}^{(t)})$ as the linear vector space consisting of all the orthogonal vectors in $V_{j}^{(t)}\in\mathbb{R}^{d\times k_j}$.  Formally, $span(V_{j}^{(t)})=\{V_{i}^{(t)}a | a \in \mathbb{R}^{k_j}\}$. Similarly, suppose $\Sigma_{ns}^{(t)}$ as $\Sigma_{ns}^{(t)}=V_{ns}^{(t)}\Lambda_{ns}^{(t)}(V_{ns}^{(t)})^{T}$, and define 
%$V_{ns}^{(t)}\in\mathbb{R}^{d\times \sum_{j\in\mathbb{U}_{ns}}k_j}$ as the concatenation of $V_{1}^{(t)},...,V_{i-1}^{(t)},V_{i+1}^{(t)},...,V_{N}^{(t)}$. 
%Then, 
$span(V_{ns}^{(t)})$ as the linear vector space consisting of all the orthogonal vectors in $V_{ns}^{(t)}$.
%$V_{1}^{(t)},...,V_{i-1}^{(t)},V_{i+1}^{(t)},...,V_{N}^{(t)}$.

Moreover, we define the domain of sensitive user $i$'s model update $x_{i}^{(t)}$ at training round $t$ as $\mathcal{X}_{i}^{(t)}$, which is a set consisting of all possible $x_{i}^{(t)}$ from user $i$. We define $\Delta \mathcal{X}_{i}^{(t)}=\{x_{i,1}^{(t)}-x_{i,2}^{(t)}|\forall x_{i,1}^{(t)}, x_{i,2}^{(t)}\in\mathcal{X}_{i}^{(t)}\}$, which consists of all the vector differences between any $x_{i,1}^{(t)}\in\mathcal{X}_{i}^{(t)}$ and $x_{i,2}^{(t)}\in\mathcal{X}_{i}^{(t)}$.
\begin{assump}[Space coverage] Assume that for any sensitive user $i$,  we have $\Delta \mathcal{X}_{i}^{(t)} \subseteq span(V_{ns}^{(t)})$. This says, for any $x_{i,1}^{(t)}\in\mathcal{X}_{i}^{(t)}$ and $x_{i,2}^{(t)}\in\mathcal{X}_{i}^{(t)}$, $x_{i,1}^{(t)}-x_{i,2}^{(t)}\in span(V_{ns}^{(t)})$.
%Then, $\forall v \in span(V_{i}^{(t)})$, we have $v \in span(V_{ns}^{(t)})$, which means there exists $A\in\mathbb{R}^{\sum_{j\in\mathbb{U}_{ns}}k_j\times k_i}$ making $V_{i}^{(t)}=V_{ns}^{(t)}A$.
\label{assum4}
\end{assump}

\begin{thm}
Under Assumption \ref{assum0},\ref{assum1},\ref{assum3},\ref{assum4}, and the assumption that each non-sensitive user $j$'s model update $x_{j}^{(t)}$ is Gaussian, the aggregated model update from other non-sensitive users $x_{ns}^{(t)}$ at step $t$ can provide $(\epsilon_i^{(t)},\delta)$-DP for sensitive user $i$, where $\epsilon_i^{(t)}=p(\lambda_{min}^{(t),*}, \delta)$ (defined in Eq. (\ref{eq:lambda1})), 
and $\lambda_{min}^{(t),*}$ is the smallest non-zero eigenvalue of $\Sigma_{ns}^{(t)}$.
\label{theorem2}
\end{thm}

\begin{proof}
Assume that $x_{i,1}^{(t)}$ and $x_{i,2}^{(t)}$ are two gradient instance of $x_{i}^{(t)}$ at step $t$, which are calculated from two local datasets $D_i^{1}$ and $D_i^{2}$ differing from one data points. Then, $\forall X \subseteq Range(x_{i}^{(t)}+x_{ns}^{(t)})$ and $\forall$ $x_{i,1}^{(t)}, x_{i,2}^{(t)} \in\mathcal{X}_{i}^{(t)}$, we have:
\begin{align}
    &\frac{Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]}{Pr[x_{i,2}^{(t)}+x_{ns}^{(t)}\in X]}\\
    =&\frac{Pr[x_{i,1}^{(t)}-x_{i,2}^{(t)}+x_{ns}^{(t)}-\mu_{ns}^{(t)}\in Y]}{Pr[x_{i,2}^{(t)}-x_{i,2}^{(t)}+x_{ns}^{(t)}-\mu_{ns}^{(t)}\in Y]}\\
    =&\frac{Pr[x_{i,1}^{(t)}-x_{i,2}^{(t)}+V_{ns}^{(t)}\Lambda_{ns}^{(t),\frac{1}{2}}n_{ns}^{(t)}\in Y]}{Pr[V_{ns}^{(t)}\Lambda_{ns}^{(t),\frac{1}{2}}n_{ns}^{(t)}\in Y]},
\end{align}
where $X=\{x - x_{i,2}^{(t)}|\forall x\in X\}$ (and $X=\{y + x_{i,2}^{(t)}|\forall y\in Y\}$). 
Due to the assumption that $x_{i,1}^{(t)}-x_{i,2}^{(t)}\in span(V_{ns}^{(t)})$, we can derive:
\begin{align}
     &\frac{Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]}{Pr[x_{i,2}^{(t)}+x_{ns}^{(t)}\in X]}\\
    =&\frac{Pr[\Lambda_{ns}^{(t),-\frac{1}{2}}(V_{ns}^{(t)})^{T}(x_{i,1}^{(t)}-x_{i,2}^{(t)})+n_{ns}^{(t)}\in Z]}{Pr[n_{ns}^{(t)}\in Z]},
\end{align}
where $Z = \{\Lambda_{ns}^{(t),-\frac{1}{2}}(V_{ns}^{(t)})^{T}y|\forall y\in Y\}$ (and $X=\{(V_{ns}^{(t)})\Lambda_{ns}^{(t),\frac{1}{2}}z|\forall z\in Z\}$ due to space coverage). 
Since:
\begin{align}
    \Delta=\max_{\forall x_{i,1}^{(t)}, x_{i,2}^{(t)}}||\Lambda_{ns}^{(t),-\frac{1}{2}}(V_{ns}^{(t)})^{T}(x_{i,1}^{(t)}-x_{i,2}^{(t)})||_2
    \leq\frac{2C}{B\sqrt{\lambda_{min}^{(t),*}}},
\end{align}
based on the proof of Theorem \ref{theorem1}, we have:
\begin{align}
    Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]
    \leq e^{\epsilon}{Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X]} + \delta,
\end{align}
where $\epsilon_i^{(t)}=p(\lambda_{min}^{(t),*}, \delta)$ (see its definition in Eq. (\ref{eq:lambda1})).
\end{proof}
\vspace{-0.1in}
\begin{corollary} (IID non-sensitive users with singular covariance matrix) 
\label{coro2}
Under Assumption \ref{assum0},\ref{assum1},\ref{assum3}, and the assumption that each non-sensitive user $j$'s model update $x_{j}^{(t)}$ is Gaussian, we further assume that all non-sensitive users’ local datasets are randomly sampled IID from a common distribution, which implies that the gradient updates of all non-sensitive users come from the identical distribution with the same mean $\mu^{(t)}$ and covariance matrix $\Sigma^{(t)}$ (i.e., $\forall j\in\mathbb{U}_{ns}$, $x_j^{(t)}\sim \mathcal{N}(\mu^{(t)}, \Sigma^{(t)})$). Let $\lambda_{min}^{(t),*}$ be the smallest non-zero eigenvalue of $\Sigma^{(t)}$. Then, the aggregated gradient from all non-sensitive users $x_{ns}^{(t)}$ at step $t$ can provide $(\epsilon_i^{(t)},\delta)$-DP for sensitive user $i\in\mathbb{U}_{s}$ with $\epsilon_i^{(t)}=\frac{2C\sqrt{2\log\frac{1.25}{\delta}}}{B\sqrt{|\mathbb{U}_{ns}|\lambda_{min}^{(t),*}}}$ for high privacy region ($\epsilon_i^{(t)}\in(0,1)$) and $\epsilon_i^{(t)}=\frac{2C^2}{B^2|\mathbb{U}_{ns}|\lambda_{0,min}^{(t),*}}$ for low privacy region ($\epsilon_i^{(t)}\geq 1$),
where $|\mathbb{U}_{ns}|$ is the number of non-sensitive users.
\end{corollary}
\begin{proof}
See Appendix \ref{sec:proof_coro2} for  details.
    % \jiang{Since $\forall j\in\mathbb{U}_{ns}, x_j^{(t)}\sim \mathcal{N}(\mu^{(t)}, \Sigma^{(t)})$, we have $\Sigma_{ns}^{(t)}=\sum_{j\in\mathbb{U}_{ns}}\Sigma_{j}^{(t)}=|\mathbb{U}_{ns}|\Sigma^{(t)}$. Hence, the smallest non-zero eigenvalue of $\Sigma_{ns}^{(t)}$ will be $|\mathbb{U}_{ns}|\lambda_{0,min}^{(t),*}$. By applying Theorem \ref{theorem2}, Corollary \ref{coro2} holds.}
\end{proof}
\vspace{-.05in}
Both Theorem \ref{theorem2} and and Corollary \ref{coro2} rely on Assumption \ref{assum4}. They state that for Gaussian model update with singular covariance matrix, in order to provide DP guarantee, any difference in individual sensitive user's model update caused by the change of one data point in their local dataset and sampling (i.e $x_{i,1 }^{(t)} - x_{i,2}^{(t)}$) must belong to the space of the randomness in the aggregated model update from other users (i.e. $span\{V_{ns}^{(t)}\}$). Otherwise, DP will be violated. The counterexample in Fig.~\ref{fig:counter_example} violates DP since the model update of user 4 fails to satisfy Assumption \ref{assum4}.

Note that Assumption \ref{assum4} can hold for IID users but may not hold for non-IID users. Moreover, in practice, it is impossible for user $i$ to verify whether Assumption \ref{assum4} holds without having access to all non-sensitive users' SVD results on the covariance matrix of their model updates. To address this problem, in Section \ref{sec:solution} we propose a practical mechanism, Water-Filling DP (WF-DP), to avoid the singularity issue of the covariance matrix in a manner that can be used in practice. Specifically, all non-sensitive users surgically add a small amount of noise to make their own covariance matrix non singular, which guarantees that their model updates will offer privacy protection to each sensitive user via the aggregation process, see Section \ref{sec:solution} for more details.

\vspace{-0.05in}
\subsection{Non-Gaussian model update}
\label{subsec:non_guassian}
Till now, our theoretical results assume that the model update from other user satisfies a Gaussian distribution (i.e. Assumption \ref{assum2}). However, this assumption may not always hold in practice for deep neural networks, as investigated in \cite{simsekli2019tail, gurbuzbalaban2021heavy}. Therefore, in this subsection, we provide DP analysis under scenarios where the model update from other users does not follow a Gaussian distribution. 
%
We start by considering the case where the model update can be approximated by a Gaussian random vector, which is formally stated as follows:
\begin{assump}[Approximately Gaussian distribution for non-sensitive users] Assume that for any set  $A\subseteq \mathrm{R}^d$, the following inequality holds:
\begin{equation}
\label{eq:assum5}
    |P(x_{ns}^{(t)}\in A) - P(n_{ns}^{(t)}\in A )|\leq \delta_0,
\end{equation}
where $n_{ns}^{(t)}\sim \mathcal{N}(\mu_{ns}^{(t)},\Sigma_{ns}^{(t)})$.
\label{assum5}
\end{assump}

%Specifically, we define $n_i^{(t)}\sim \mathcal{N}(\mu_i^{(t)},\Sigma_i^{(t)})$ as a Gaussian random vector with mean $\mu_i^{(t)}$ and covariance matrix $\Sigma_i^{(t)}$. And we define $n_{ns}^{(t)}\sim \mathcal{N}(\mu_{ns}^{(t)},\Sigma_{ns}^{(t)})$, which is a Gaussian random vector with mean $\mu_{ns}^{(t)}$ and covariance matrix $\Sigma_{ns}^{(t)}$. Then, 
\begin{assump}[Non-singluar covariance matrix  for non-sensitive users] Assume that for any non-sensitive user $j\in\mathbb{U}_{ns}$, its gradient update has non-singluar covariance matrix, which means the smallest eigenvalue of $\Sigma_j^{(t)}$ is non-zero.
\label{assum6}
\end{assump}

Under the above assumptions, we can prove Theorem \ref{theorem3} and Theorem \ref{theorem4} below:
\begin{thm}
Under Assumption \ref{assum0},\ref{assum1} and Assumption \ref{assum5},\ref{assum6}, the aggregated gradient from non-sensitive users $x_{ns}^{(t)}$ at step $t$ can provide $(\epsilon_i^{(t)},\delta+\delta_c)$-DP for sensitive user $i$, where $\epsilon_i^{(t)}=p(\lambda_{min}^{(t)},\delta)$, and $\lambda_{min}^{(t)}$ is the smallest eigenvalue of $\Sigma_{ns}^{(t)}$, $\delta_c=(1+e^{\epsilon_i^{(t)}})\delta_0$.
\label{theorem3}
\end{thm}
\begin{proof}
See Appendix \ref{sec:proof_theorem3} for details.
\end{proof}
% Assume that $x_{i,1}^{(t)}$ and $x_{i,2}^{(t)}$ are two gradient instance of $x_{i}^{(t)}$ at step $t$, which are calculated from two local datasets $D_i^{1}$ and $D_i^{2}$ differing from one data points. Then, $\forall X \subseteq Range(x_{i}^{(t)}+x_{ns}^{(t)})$ and $\forall$ $x_{i,1}^{(t)}$ and $x_{i,2}^{(t)}$,  we have:
% \begin{align}
%     & Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X] - e^{\epsilon_i^{(t)}}Pr[x_{i,2}^{(t)}+x_{ns}^{(t)}\in X]\\
%     \leq & (Pr[x_{i,1}^{(t)}+n_{ns}^{(t)}\in Z] + \delta_0) - e^{\epsilon_i^{(t)}}(Pr[x_{i,2}^{(t)}+n_{ns}^{(t)}\in Z]-\delta_0)\\
%     \leq & Pr[x_{i,1}^{(t)}+n_{ns}^{(t)}\in Z] - e^{\epsilon_i^{(t)}}Pr[x_{i,2}^{(t)}+n_{ns}^{(t)}\in Z] + (1+e^{\epsilon_i^{(t)}})\delta_0.
% \end{align}
% where $n_{ns}^{(t)}\sim N(\mu_{ns}^{(t)},\Sigma_{ns}^{(t)})$ is a Gaussian random vector. Based on Theorem \ref{theorem1}, we have:
% \begin{align}
%     Pr[x_{i,1}^{(t)}+n_{ns}^{(t)}\in Z] - e^{\epsilon_i^{(t)}}Pr[x_{i,2}^{(t)}+n_{ns}^{(t)}\in Z]\leq\delta.
% \end{align}

% Hence, we can derive:
% \begin{align}
%     & Pr[x_{i,1}^{(t)}+x_{ns}^{(t)}\in X] - e^{\epsilon_i^{(t)}}Pr[x_{i,2}^{(t)}+x_{ns}^{(t)}\in X]\\
%     \leq & \delta + (1+e^{\epsilon_i^{(t)}})\delta_0
%     = \delta + \delta_c.
% \end{align}
\begin{thm}
Under Assumption \ref{assum0},\ref{assum1}, and Assumption \ref{assum3}, \ref{assum4}, \ref{assum5}, 
the aggregated gradient from other users $x_{ns}^{(t)}$ at step $t$ can provide $(\epsilon_i^{(t)},\delta+\delta_c)$-DP for user $i$, where $\epsilon_i^{(t)}=p(\lambda_{min}^{(t),*},\delta)$,  $\lambda_{min}^{(t),*}$ is the smallest non-zero eigenvalue of $\Sigma_{ns}^{(t)}$, $\delta_c=(1+e^{\epsilon_i^{(t)}})\delta_0$.
\label{theorem4}
\end{thm}
\begin{proof}
    Theorem \ref{theorem4} can be directly proved by combing the proofs for Theorem \ref{theorem2} and \ref{theorem3}.
\end{proof}

Both Theorem \ref{theorem3} and Theorem \ref{theorem4} state that if the model update from all non-sensitive users is approximately a Gaussian distribution, it can still provide $(\epsilon,\delta)$-DP guarantee for any sensitive users, where only the $\delta$ will be affected compared with Theorem \ref{theorem1} and Theorem \ref{theorem2} under the Gaussian model update assumption.

\medskip
\noindent\textbf{Remark 1: Applicability of Assumption \ref{assum5} in practice.} 
The rationale of Assumption \ref{assum5} comes from Central Limit Theorem (CLT). Since the model update in FedSGD is commonly an average of $B$ gradients calculated from $B$ data points sampled independently from an identical distribution (i.i.d), if CLT holds in this application, the model update is expected to converge to a Gaussian random vector \cite{shang2015covariance,zhu2018anisotropic, mandt2017stochastic} as the batch size $B$ increase.

%The gradient update from user $i$ at step $t$, $x_i^{(t)}$, can be viewed as the average of $B$ independent gradient $g_i(\bm{\theta^{(t)}},b)$ from the same distribution with mean $\mu_i^{(t)}$ and $\Sigma_i^{(t)}$. Based on the Multivariable Berry-Esseen theorem, if the third moment of $g_i(\bm{\theta^{(t)}},b)$ is bounded, then as $B$ goes to infinity, $x_i^{(t)}$ will converge to a Gaussian random vector, which means Assumption \ref{assum6} will hold. 
However, there are two issues for Assumption \ref{assum5} to hold in practice. Firstly, recent works such as \cite{simsekli2019tail, gurbuzbalaban2021heavy} have found that the Gaussian assumption about stochastic noise may fail to hold in deep learning settings, due to the violation of finite-variance assumption in CLT. 
Secondly, perhaps more importantly, in order to make the $\delta+\delta_c$ in Theorem \ref{theorem3} meaningful, $\delta_0$ in~\eqref{eq:assum5} in Assumption \ref{assum5} needs to be at least smaller than $1/|D_i|$, which is non-trivial. While the Multivariable Berry-Esseen Theorem \cite{raivc2019multivariate} provides a general bound for the CDF (cumulative distribution function) difference between the sum of $B$ i.i.d sampled random vectors and a Gaussian random vector (i.e. the left part of~\eqref{eq:assum5} in Assumption \ref{assum5}), no prior works have revealed the convergence rate of this bound w.r.t $B$ on a general set $A$. In other words, it has not been proven that $\delta_0$ can converge to zero (or become smaller enough) as we increase $B$. Therefore, there is a lack of practical methods to determine the batch size $B$, such that we can guarantee that $\delta_0$ is small enough for achieving DP with meaningful $\delta$.  
% Hence, we cannot prove that non-Gaussian gradient in FedSGD can provide $(\epsilon,\delta)$-DP with meaningful $\delta$ in practice. 

%\medskip
%\noindent\textbf{Practical solution.} 
As a practical solution to provide DP guarantee in the non-Gaussian model update scenarios, users can choose to replace their original model update with a Gaussian random vector, which is sampled from a multivariate Gaussian distribution with the same mean $\mu_i^{(t)}$ and covariance matrix $\Sigma_i^{(t)}$ as the original model update. While in theory this may introduce model inaccuracies, in Section \ref{sec:eval}, where we evaluate the privacy guarantee and the model performance under various scenarios using real world datasets, we show that in practice there is minimal performance penalty.
Along the same lines,  
researchers in \cite{wu2020noisy} have also demonstrated that Gaussian gradient noise can achieve comparable performance compared with the inherent stochastic gradient noise. 
Motivated by the above, 
our proposed WF-DP mechanism introduced in 
Section \ref{sec:solution}
does replace the original model updates of users with a Gaussian random vector, see Section \ref{sec:solution} for more details.

\noindent\textbf{Remark 2: Generalization to other FL protocols.}
% \label{sec:fedavg}
While our theoretical results are derived based on FedSGD, they can be generalized to other FL algorithms such as FedAvg \cite{mcmahan2017communication}, by only varying how we generate the model update (i.e. Assumption \ref{assum1}). As an example, in FedAvg, at training round $t$ each user conducts multiple local training steps (i.e. a random process) to derive their local model update $x_{i}^{(t)}$, which will also be a random vector with some mean and covariance matrix. Therefore, after changing Assumption \ref{assum1} w.r.t. how we generate $x_{i}^{(t)}$, Theorem \ref{theorem1}-\ref{theorem4} can be directly applied. 
% Note that in FedAvg, we do not have the sampling ratio $q_{i}^{(t)}$ for DP amplification. Instead, we can amplify DP via user selection (i.e. randomly select a subset of users in each training round) \cite{zhang2022understanding}. 

\noindent\textbf{Remark 3: DP noise for sensitive users. } It is worth noting that the DP noise for each sensitive user is a function of the data distribution of the other non-sensitive users, not the data distribution of the sensitive users we want to protect. From the perspective of each sensitive user, the other non-sensitive users’ model update can serve as an independent Gaussian random vector, which can provide ($\epsilon,\delta$)-DP for all worst-case datasets of the sensitive user. Specifically, the $\epsilon$ value for each sensitive user is bounded by the minimal eigenvalue of the covariance matrix from the other non-sensitive users, regardless of his/her own data distribution. We acknowledge that the value of $\epsilon$ is not controlled by the sensitive users but it does nevertheless guarantee DP at that level.



